Training Kinetics in 15 Minutes: Large-scale Distributed Training on Videos

Deep video recognition is more computationally expensive than image recognition, especially on large-scale datasets like Kinetics [1]. Therefore, training scalability is essential to handle a large amount of videos. In this paper, we study the factors that impact the training scalability of video networks. We recognize three bottlenecks, including data loading (data movement from disk to GPU), communication (data movement over networking), and computation FLOPs. We propose three design guidelines to improve the scalability: (1) fewer FLOPs and hardware-friendly operator to increase the computation efficiency; (2) fewer input frames to reduce the data movement and increase the data loading efficiency; (3) smaller model size to reduce the networking traffic and increase the networking efficiency. With these guidelines, we designed a new operator Temporal Shift Module (TSM) that is efficient and scalable for distributed training. TSM model can achieve 1.8x higher throughput compared to previous I3D models. We scale up the training of the TSM model to 1,536 GPUs, with a mini-batch of 12,288 video clips/98,304 images, without losing the accuracy. With such hardware-aware model design, we are able to scale up the training on Summit supercomputer and reduce the training time on Kinetics dataset from 49 hours 55 minutes to 14 minutes 13 seconds, achieving a top-1 accuracy of 74.0%, which is 1.6x and 2.9x faster than previous 3D video models with higher accuracy. The code and more details can be found here: http://tsm-hanlab.mit.edu.

==> figureText/tab_scalability.tex <==
\renewcommand \arraystretch{1}
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\caption{Detailed statistics about scalability. We can train a TSM model within 15 minutes and achieve 74\% top-1 accuracy.}
\label{tab:scalability}
\small
\begin{center}
\begin{tabular}{llllll}
\toprule
\textbf{\#Node} &  \textbf{\#GPU} &  \textbf{BatchSize} & \textbf{\#Frame} &  \textbf{Accuracy} & \textbf{Time}\\
\midrule
1 & 6 & 48 & 384 & - & 49h 55m \\ 
\hline
16 & 96 & 768 & $6k$ & 74.18$\pm$0.14 & 3h 38m \\
32 & 192 & $1.5k$ & $12k$ & 74.14$\pm$0.10 & 1h 50m  \\
64 & 384 & $3k$ & $25k$ & 74.10$\pm$0.08 & 55m 56s \\
128 & 768 & $6k$ & $49k$ & 73.99$\pm$0.04 & 28m 14s \\
\textbf{256} & $\mathbf{1.5k}$ & $\mathbf{12k}$ & $\mathbf{98k}$ & \textbf{73.99$\pm$0.07} & \textbf{14m 13s} \\
\midrule
384 & $2.3k$ & $18k$ & $147k$ & 69.80$\pm$0.13 & 10min 9s \\ 
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> figureText/tab_training_cost.tex <==
\renewcommand \arraystretch{1}
\begin{table}[t]
\setlength{\tabcolsep}{3pt}
\caption{Comparing the training cost of image and video recognition model.\SH{I3D and TSM have the same amount of forward FLOPs? due to pooling?}\LJ{The computation is not an order of magnitude larger? Should we still put this table?}\SH{maybe not. TSM doesn't save FLOPs than I3D, due to pooling?}}
% \vspace{-6pt}
\label{tab:training_cost}
\small
\begin{center}
\begin{tabular}{cccccc}
\toprule
 \multirow{2}{*}{\textbf{Dataset}} &  \multirow{2}{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Factors}} & \multirow{2}{*}{\textbf{\shortstack{Total\\FLOPs}}}  \\  \cmidrule(lr){3-5}
 & & \shortstack{Forward\\FLOPs} & \shortstack{Train\\Epochs} &  \shortstack{Trainset\\Size} & \\
\midrule
ImageNet & Res50 & 4G & 90 & 1.28M & 4.6e+17\\
\midrule
Kinetics-400 & Res50 TSM\textsubscript{8f} & 33G & 100 & 0.25M & 8.3e+17 \\
Kinetics-400 & Res50 I3D~\cite{wang2017non} & 33G & 100 \\
Kinetics-400 & Res50 TSM\textsubscript{16f} & 65G & 100 & 0.25M \\
Kinetics-600 & Res50 TSM\textsubscript{8f} & & 100 & 0.39M \\
Kinetics-700 & Res50 TSM\textsubscript{8f} & & 100 & 0.55M \\
\bottomrule
\end{tabular}
\end{center}
% \vspace{-15pt}
\end{table}

% 246,535
% 
